Generalized Deduplication: Bounds, Convergence, and Asymptotic Properties

We study a generalization of deduplication, which enables lossless deduplication of highly similar data and show that standard deduplication with fixed chunk length is a special case. We provide bounds on the expected length of coded sequences for generalized deduplication and show that the coding has asymptotic near-entropy cost under the proposed source model. More importantly, we show that generalized deduplication allows for multiple orders of magnitude faster convergence than standard deduplication. This means that generalized deduplication can provide compression benefits much earlier than standard deduplication, which is key in practical systems. Numerical examples demonstrate our results, showing that our lower bounds are achievable, and illustrating the potential gain of using the generalization over standard deduplication. In fact, we show that even for a simple case of generalized deduplication, the gain in convergence speed is linear with the size of the data chunks.

==> sections/objects/dedupeqfig.tex <==
%\begin{figure*}[!t]
%%\normalsize
%%\setcounter{tempeqcounter}{\value{equation}} % temp store of current value
%\begin{IEEEeqnarray}{rCl}
%\setcounter{equation}{1}
%%\setcounter{equation}{\value{storeeqcounter_one}} % number of this equation
%~C &+& \sum\limits_{c=1}^{C} \Big[ n \left(1 - |\mathcal{Z}|^{-1}\right)^{c-1}
% + \left(1 - \left(1 - |\mathcal{Z}|^{-1}\right)^{c-1}\right) \log \left(|\mathcal{Z}|\left(1 - \left(1 - |\mathcal{Z}|^{-1}\right)^{c-1}\right)\right) \Big]  \nonumber\\
%&\leq &R_D(C) \leq ~2C + \sum\limits_{c=1}^{C} \Big[ n \left(1 - |\mathcal{Z}|^{-1}\right)^{c-1} 
%+ |\mathcal{Z}|^{-1} \min\{ (c-1) \log(c-1) , |\mathcal{Z}|\log|\mathcal{Z}|\}\Big].
%\label{eq:deduplicationBoundsThm}
%\end{IEEEeqnarray}
%%\setcounter{equation}{\value{tempeqcounter}} % restore correct value
%%\hrulefill
%\vspace*{-10pt}
%\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
\vspace*{-0.45cm}
%\normalsize
%\setcounter{tempeqcounter}{\value{equation}} % temp store of current value
\begin{IEEEeqnarray}{rCl}
\setcounter{equation}{3}
%\setcounter{equation}{\value{storeeqcounter_one}} % number of this equation
L_D(C) &=& C + \sum\limits_{c=1}^{C} \Big[ n \left(1 - |\mathcal{Z}|^{-1}\right)^{c-1}
 + \left(1 - \left(1 - |\mathcal{Z}|^{-1}\right)^{c-1}\right) \log \left(|\mathcal{Z}|\left(1 - \left(1 - |\mathcal{Z}|^{-1}\right)^{c-1}\right)\right) \Big] \label{eq:deduplicationBoundsThm1}\\
U_D(C) &=& 2C + \sum\limits_{c=1}^{C} \Big[ n \left(1 - |\mathcal{Z}|^{-1}\right)^{c-1} 
+ |\mathcal{Z}|^{-1} \min\{ (c-1) \log(c-1) , |\mathcal{Z}|\log|\mathcal{Z}|\}\Big]
\label{eq:deduplicationBoundsThm2}
\end{IEEEeqnarray}
%\setcounter{equation}{\value{tempeqcounter}} % restore correct value
\hrulefill
\vspace*{-10pt}
\end{figure*}

==> sections/objects/geneqfig.tex <==
%\begin{figure*}[!t]
%%\normalsize
%%\setcounter{tempeqcounter}{\value{equation}} % temp store of current value
%\begin{IEEEeqnarray}{rCl}
%%\setcounter{equation}{\value{storeeqcounter_two}} % number of this equation
%\setcounter{equation}{2}
%C(\log|\mathcal{Y}|+1)& + &\sum\limits_{c=1}^{C} \left[ k \left(1 - |\mathcal{X}|^{-1}\right)^{c-1}  + \left(1 - \left(1 - |\mathcal{X}|^{-1}\right)^{c-1}\right) \log \left( |\mathcal{X}| \left( 1 - \left( 1 - |\mathcal{X}|^{-1}\right)^{c-1}\right)\right) \right]\nonumber\\
%& \leq &R_G(C) \leq C(\log\mathcal{|Y|}+3) + \sum\limits_{c=1}^{C} \left( k \left(  1 - |\mathcal{X}|^{-1}\right)^{c-1} + |\mathcal{X}|^{-1} \min\{ (c-1) \log(c-1) , |\mathcal{X}|\log|\mathcal{X}|\}\right).
%\label{eq:generalizedBoundsThm}
%\end{IEEEeqnarray}
%%\setcounter{equation}{\value{tempeqcounter}} % restore correct value
%\hrulefill
%\vspace*{0pt}
%\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure*}[!t]
%\hrulefill
%%\normalsize
%%\setcounter{tempeqcounter}{\value{equation}} % temp store of current value
%\begin{IEEEeqnarray}{rCl}
%%\setcounter{equation}{\value{storeeqcounter_two}} % number of this equation
%\setcounter{equation}{1}
%L_G(C) &=& C(\log|\mathcal{Y}|+1) + \sum\limits_{c=1}^{C} \left[ k \left(1 - |\mathcal{X}|^{-1}\right)^{c-1}  + \left(1 - \left(1 - |\mathcal{X}|^{-1}\right)^{c-1}\right) \log \left( |\mathcal{X}| \left( 1 - \left( 1 - |\mathcal{X}|^{-1}\right)^{c-1}\right)\right) \right]\label{eq:generalizedBoundsThm1}\\
%U_G(C) &=& C(\log\mathcal{|Y|}+3) + \sum\limits_{c=1}^{C} \left( k \left(  1 - |\mathcal{X}|^{-1}\right)^{c-1} + |\mathcal{X}|^{-1} \min\{ (c-1) \log(c-1) , |\mathcal{X}|\log|\mathcal{X}|\}\right)
%\label{eq:generalizedBoundsThm2}
%\end{IEEEeqnarray}
%%\setcounter{equation}{\value{tempeqcounter}} % restore correct value
%\hrulefill
%\vspace*{0pt}
%\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
\hrulefill
%\normalsize
%\setcounter{tempeqcounter}{\value{equation}} % temp store of current value
%\setcounter{equation}{\value{storeeqcounter_two}} % number of this equation
\setcounter{equation}{0}
\begin{IEEEeqnarray}{rCl}
L_G(C, \mathcal{X}, \mathcal{Y}) &=& C(\log|\mathcal{Y}|+1) + \sum\limits_{c=1}^{C} \left[ k p_{\mathcal{X}}(c)  + \left(1 - p_{\mathcal{X}}(c)\right) \log \left(1 - p_{\mathcal{X}}(c)\right) \right],\label{eq:generalizedBoundsThm1}\\
U_G(C, \mathcal{X}, \mathcal{Y}) &=& C(\log\mathcal{|Y|}+3) + \sum\limits_{c=1}^{C} \left[ k p_{\mathcal{X}}(c) + |\mathcal{X}|^{-1} \min\{ (c-1) \log(c-1) , |\mathcal{X}|\log|\mathcal{X}|\}\right]. \label{eq:generalizedBoundsThm2}
\end{IEEEeqnarray}
%\setcounter{equation}{\value{tempeqcounter}} % restore correct value
\hrulefill
\vspace*{0pt}
\end{figure*}

